Intrusive acceleration strategies for Uncertainty Quantification for hyperbolic systems of conservation laws

Methods for quantifying the effects of uncertainties in hyperbolic problems can be divided into intrusive and non-intrusive techniques. Non-intrusive methods allow the usage of a given deterministic solver in a black-box manner, while being embarrassingly parallel. However, avoiding intrusive modifications of a given solver takes away the ability to use several inherently intrusive numerical acceleration tools. Moreover, intrusive methods are expected to reach a given accuracy with a smaller number of unknowns compared to non-intrusive techniques. This effect is amplified in settings with high dimensional uncertainty. A downside of intrusive methods is however the need to guarantee hyperbolicity of the resulting moment system. In contrast to stochastic-Galerkin (SG), the Intrusive Polynomial Moment (IPM) method is able to maintain hyperbolicity at the cost of solving an optimization problem in every spatial cell and every time step. In this work, we propose several acceleration techniques for intrusive methods and study their advantages and shortcomings compared to the non-intrusive Stochastic Collocation method. When solving steady problems with IPM, the numerical costs arising from repeatedly solving the IPM optimization problem can be reduced by using concepts from PDE-constrained optimization. Additionally, we propose an adaptive implementation and efficient parallelization strategy of the IPM method. The effectiveness of the proposed adaptations is demonstrated for multi-dimensional uncertainties in fluid dynamics applications, resulting in the observation of requiring a smaller number of unknowns to achieve a given accuracy when using intrusive methods. Furthermore, using the proposed acceleration techniques, our implementation reaches a given accuracy faster than Stochastic Collocation.

==> colloc_ipm.tex <==
%\subsection{Collocation accelerated IPM}
%\label{sec:collIPM}
%Commonly, a great amount of iterations in pseudo-time is needed to converge to a steady state solution. Consequently, the IPM method which requires solving the dual problem \eqref{eq:dualProblem} in every spatial cell in each iteration becomes prohibitively expensive. We tackle this problem by using IPM only as a postprocesssing step for the steady solution obtained by a cheap method. (Or vice-versa, we use a cheap method as a preprocessing step for IPM). In our case, we perform the preprocessing step with stochastic-Collocation, i.e. we converge the moments to a steady state solution by applying collocation steps. The obtained moments are then used as initial condition for the IPM moment system (for which the moments are no longer a steady state solution). After applying a significantly reduced number of IPM iterations, we obtain a steady state IPM solution. In our numerical experiments presented in section \ref{sec:results}, we can show that the overall costs are dominated by the large number of cheap collocation steps and not by the small number of expensive IPM steps, while the solution shows the expected desirable properties of the IPM solution.

%Different variants of this method are possible:
%\begin{itemize}
%\item Since the IPM iterations will again modify the steady state Collocation solution, it is not necessary to converge Collocation to the exact steady state solution before starting IPM. Here, one needs to determine an indicator to choose at which residual the collocation iteration is sufficiently accurate and can therefore be switched to IPM.
%\item The main idea is to use a cheap but inexact method as a preconditioner for an expensive but accurate method. Here, one is not limited in choosing SC and IPM, but one can for example choose Monte Carlo methods as an accelerator or SC with an increased number of quadrature points as the expensive method. Note that in the latter case, a map from the moments to the solution at the increased quadrature set is required, for which the IPM reconstruction \eqref{eq:ansatz} would be a suitable choice.
%\end{itemize}
